Measuring Attribution in Natural Language Generation Models

With recent improvements in natural language generation (NLG) models for various applications, it has become imperative to have the means to identify and evaluate whether NLG output is only sharing verifiable information about the external world. In this work, we present a new evaluation framework entitled Attributable to Identified Sources (AIS) for assessing the output of natural language generation models, when such output pertains to the external world. We first define AIS and introduce a two-stage annotation pipeline for allowing annotators to appropriately evaluate model output according to AIS guidelines. We empirically validate this approach on generation datasets spanning three tasks (two conversational QA datasets, a summarization dataset, and a table-to-text dataset) via human evaluation studies that suggest that AIS could serve as a common framework for measuring whether model-generated statements are supported by underlying sources. We release guidelines for the human evaluation studies.

==> AIS Paper (Arxiv Copy) - July 19, 2022/sections/background.tex <==
\section{Background}\label{sec:background}
\textbf{Hallucations in NLG.} As alluded to in \S\ref{sec:intro}, past work has identified the issue of hallucination in neural generation models.
\newcite{wiseman-etal-2017} presented challenges in data-to-text generation where neural models generate hallucinated content not supported by source data;  they proposed an automatic information extraction-based metric to evaluate generated text for that particular scenario and conducted a small human evaluation study examining whether summaries are supported by source data.
More recently, \newcite{parikh-etal-2020-totto} presented a larger human evaluation study in the context of a data-to-text generation dataset entitled ToTTo, and measured hallucinations in terms of \textit{faithfulness} with respect to a source data table.

Hallucination has been a salient subject of investigation in text summarization. \newcite{maynez2020faithfulness} presented an extensive characterization of hallucinations, discussed behavior of models that generate content that are present in larger corpora beyond a given source and conducted a significant human study. Additional automatic QA-based methods for detecting hallucinations have been proposed by \newcite{wang-etal-2020-asking}, \newcite{nan-etal-2021-improving}, among others.
One of the most relevant papers, \newcite{durmus-etal-2020-feqa}, involved both a human evaluation and the introduction of an automatic question--answer based evaluation method. Their human evaluation of summary sentences is similar to our two-stage annotation pipeline where they evaluate sentences in two steps --- first for whether it is understandable, and second, if so, for faithfulness to the underlying source (their instructions to annotators are: ``If the information conveyed by the sentence is not expressed in the source, select `unfaithful'.'').  



In the case of response generation for dialogue, especially in scenarios that involve the system responding about the real world, research has focused on measuring the responses' consistency to prior conversational history or their groundedness to some external evidence, that we deem to be very close to the topic of hallucination.
These have been measured via dialogue-specific natural language inference methods, often via human studies and data creation \cite{Welleck2019DialogueNL,mehri-eskenazi-2020-usr,Gupta2021DialFactAB,Honovich2021Q2EF,Dziri2021EvaluatingGI,santhanam2021rome}.

Despite a significant amount of work pertaining to hallucination spanning multiple NLG problems, there is no unified approach to evaluate whether system generated statements are supported by underlying source documents.
Human evaluation studies are varied from paper to paper and detailed, reproducible annotation instructions are unavailable \cite{belz2020disentangling}. Likewise, the use of terminology for describing and defining evaluation criteria also lacks consistency and further complicates reproducibility \cite{howcroft2020twenty}.
General-purpose benchmarking across these tasks have gained traction \cite{gehrmann-etal-2021-gem}, but there has not been a standardized treatment of the attribution problem.
Our paper attempts to address this gap by explicitly formalizing the evaluation of attribution as a replicable and extendable conceptual framework.  As part of our definition of attribution, we outline a more formal background for ``information conveyed by the text'' --- in particular through the use of explicatures (see Figure~\ref{fig:explicatures} for examples). Lastly, we demonstrate that AIS can be generalized across multiple NLG tasks in which context, source documents, and generated text can take different forms. 




\noindent\textbf{Fact Verification.} A related field of study has dealt with the topic of fact or claim verification \cite[\textit{inter alia}]{thorne-etal-2018-fever,Thorne2018AutomatedFC,DBLP:journals/corr/abs-2104-00640}.
Work in this area has framed the task as retrieving supporting evidence given a claim, and optionally classifying semantic relationships between the claim and the evidence text.
Modeling approaches have overlapped with recent literature examining natural language inference \cite{DBLP:conf/aaai/NieCB19}.
\citet{DBLP:journals/corr/abs-2104-00640} have examined several human annotation tasks for the above family of problems;  however, there are several key differences with this work. First, we evaluate the quality of a system generated utterance with respect to given evidence source (a fundamentally different end goal); we utilize the notion of explicatures in defining attribution; finally, we avoid absolute judgments regarding ``factuality'' of utterances.
As mentioned in \S\ref{sec:intro}, rather than making  factuality judgments, we deem that complementary evaluation methods such as ``source quality'' in tandem with AIS would be required to evaluate the factuality of utterances.
As a corollary, we assume the source is a reference, and that an actual system may select sources for their trustworthiness.

\noindent \textbf{Decontextualization.} \citet{choi2021decontext} introduce the task of decontextualization, that is, the problem of taking a sentence in context and rewriting it in a way that it's meaning is preserved, and it can be interpreted out of context. This is directly related to the idea of explicatures, which are also used in the current paper. 


==> AIS Paper (Arxiv Copy) - July 19, 2022/sections/discussion.tex <==
\section{Discussion}

Generative models have been advancing toward human-like competence in some aspects. Their real-world application in consumer-focused information products are becoming more attractive, for example, for summarizing original descriptions of events, or for deriving answers to pertinent questions about the world. Traditionally, this type of information transformation has been performed by specialized human experts (e.g., journalists, researchers), who are required to meet a variety of standards of accuracy and accountability, maintaining one or more sources for a proposition and performing fact-checking. The task could also be likened to the practice of law, where norms are examined for their subsumptive relationship to a set of circumstances, and where both close reading and a set of conventionalized tests aid this determination.

We formalize a specific sub-task of fact-checking, namely, verification against a known source, as a necessary but not sufficient step in ensuring the quality of generated text. We show that with the right training, careful instructions, and optimized user interfaces, we can delegate the judgment of attribution to underlying source(s) to crowd workers, but we also find limitations. Following the data collection we described, we found it necessary to set some standards in our instructions to raters. This includes setting expectations for named entities, for example, whether first and last names are needed to identify an individual and to link them between evidence and statement, or if a place name without qualification may be acceptable as long as there are no other well-known places of the same name. Similarly, as statements and evidence become more complex, raters inevitably draw inferences using individual world knowledge. This is unavoidable and is inherently noisy \cite{pavlick2019inference}; ground truth is ambiguous, just like journalists, researchers, or judges often legitimately disagree. Possible model outputs fall on a spectrum ranging from synthesized information to the mostly unassailable extractive generations \cite{ladhak2022faithful}. AIS does not set policy about where model output should fall: its users still need to decide where to draw the line.

AIS is limited to propositions that can be judged with the "according to" framework. AIS is not applicable to questions (without presuppositions) or imperatives (commands and requests). There are also scenarios where strict attribution contradicts other desirable output characteristics (e.g., chit--chat systems). We did not examine AIS on such data. How to evaluate hybrid systems that mix entertaining and informative communicative goals --- capturing the attribution of the informative portion but ignoring the rest --- is unclear, as is the question of whether systems with blurry boundaries between what is and is not subject to attribution should exist at all. 

We have purposefully limited the availability of context in our definition. Practical human--computer interactions may actually take place in context beyond the shared time $t$ that is used in the definition (Section~\ref{sec:definitions}), perhaps because the communication channel is richer than a text-based line of transmission, and because it may be further extended by multi-session interaction history. It is important that annotators remain aware of the notion of explicature, resolving explicit references and implicit topics available to the communicators. It is possible that the use of models that perform this task \cite{choi2021decontext} can improve the performance of raters. We are also aware that this task requires close reading, which is challenging to implement on crowdsourcing platforms where speed, efficiency, and cost are incentivized instead. Again, models may be useful in extracting explicit, elementary propositions from complex statements, making this task easier for raters. We will examine such approaches in future work.


==> AIS Paper (Arxiv Copy) - July 19, 2022/sections/experiments.tex <==
\section{Experiments}
\label{sec:task-results}
In the following section, we demonstrate the utility of the AIS templates by showing how it can be applied to three different tasks (conversational QA, summarization, and table-to-text generation) in which the model output is --- by design --- always meant to be attributable to some source document.  We  instantiated the AIS annotation template for four datasets in these domains (see Table~\ref{tab:tasks}) and performed human evaluation studies on generated outputs from multiple models. In order to show the applicability of AIS in detecting nuanced differences between different types of model outputs, we specifically chose models for each dataset that would represent a range of different types of outputs rather than just selecting a set of state-of-the-art models.  We also annotated a selection of gold references from each dataset to better understand the AIS quality of existing datasets in these areas.  We end with analysis of how effectively humans can annotate AIS as well as a discussion of various interpretability and AIS patterns that we found in the resulting annotations.
\input{tables/tasks_table}

\subsection{QReCC Answer Generation}
\paragraph{Set-up} We use the QReCC dataset \cite{qrecc}, a collection of multi-turn conversational QA interactions that extends conversations coming from NaturalQuestions \cite{NQppr}, QUAC \cite{quacppr}, and CAST-19 \cite{castppr}.  In this task, a model is given a conversational history and generates a contextualized response.  We use a task set-up where the document passage containing the answer to the current query has already been retrieved (using the oracle retrieved document passage as the attributed source). We use different variations of T5 models including both base and small size variants.  First, we use the pre-trained T5 models (PT) by themselves by prompting the model (formatted as: ``Query:... Conversation History: ... Document: ... Answer:'').  We also use a version of T5 that has been fine-tuned on QReCC (FT) which uses special tokens to separate the query, context, and document instead of natural-language prompts.  Lastly, to sanity-check the AIS measures, we use a version of the model (no evidence) that only sees the query and conversation history but not the document at generation time.  We expect that the AIS subscores should be much lower in the model that does not use the evidence from document to generate the answer.
 
\input{tables/qrecc_results_table}
\paragraph{Results} We show results in Table~\ref{tab:qrecc}. The model outputs' interpretability increases substantially after fine-tuning (by about 50 points).  The AIS subscore is  highest in the fine-tuned model that uses evidence in its input.  As expected, the AIS is drastically lower in the model that does not use the document as input at generation time (the no evidence model) which is both interpretable and AIS only 15\% of the time.  Differences between model sizes (small vs. base) are generally not significant except for the pretrained-only model, though the AIS scores of the smaller versions are typically slightly higher.  


\subsection{WoW Answer Generation}
\paragraph{Set-up} We used the seen portion of the test set from Wizard of Wikipedia \cite{dinan2019wizard}.  In this task, a model is given a conversational history and generates a contextualized response based on information from Wikipedia. As with QReCC, we again use a set-up where the Wikipedia sentence has already been retrieved (using the oracle retrieved sentence as the attributed source). To avoid chit--chat style utterances that may not be sharing new information, we sampled 200 examples per model where the previous utterance was a question (contains `?').  We used the models from \citet{rashkinetal}. That paper introduced a controlled T5 model trained on the Wizard of Wikipedia data which uses control tags and re-sampling to target generations that are more faithful to the document (by looking at heuristics such as entailment metrics, lexical precision, and first-person usage). Similar to that paper, we also compared with three models that are seq2seq-style conversation models: the original answer generation system from \citet{dinan2019wizard}, the Dodecadialogue multitask system from \citet{dodeca} and a T5-base model \citep{t5ppr} finetuned on Wizard of Wikipedia data. Because the model from \citet{rashkinetal} was specifically trained to be more faithful to evidence, we expect that it will score higher in the AIS category.

\input{tables/wow_results_table}
\paragraph{Results} We show results in Table~\ref{tab:wow}.  Compared to the QReCC data (in which only a few examples were flagged), more examples were flagged with the Wizard of Wikipedia data, which we included as an extra column.  The general trend of results is similar to what was found in the human evaluations of faithfulness and subjectivity in \citet{rashkinetal}.  As expected, the model that has specific controllable inputs for increasing the model's faithfulness to the input document achieves the highest the AIS scores overall.  We also note that the AIS scores of the gold references is lower than the model outputs.  We discuss this more in Section~\ref{sec:goldref}.

\subsection{CNN/DM Summarization}
\paragraph{Set-up} We extend our evaluation framework for a second task, summarization to confirm that AIS can be more broadly applicable.  AIS is crucial in summarization where a generated summary ($S$) must be well-supported by the source article ($P$). In contrast to some of the prior work in hallucination evaluation in summarization \citep{durmus-etal-2020-feqa,maynez2020faithfulness}, the annotators in our task evaluate the full summary for attribution (rather than at a sentence-level or a span-level), in order to account for cases where two individual text spans may be attributable to a source document but --- when composed together --- convey information that is different from the source document (e.g.,  misordered events, pronouns that no longer have the correct references when misordered, etc.). As a first step in applying AIS to summarization, we compare the performance of three different approaches (abstractive vs. extractive vs. hybrid) on 200 examples randomly sampled from the CNN/DM \citep{cnndm} test set.  The source articles in this dataset come from articles in CNN and DailyMail news and the summaries are extracted from bulleted highlights that were included with the article by the journalists.  We expect that high-quality AIS annotations will show a trend where extractive systems achieve higher AIS scores because they are copying directly from the source without adding anything. First, we used MatchSum \citep{matchsum}, a state-of-the-art extractive summarization model.  Because this model is extractive, it is expected that it will be the least prone to hallucinations.  We also used an abstractive summarization system, BigBird \citep{bigbird}.  Lastly, we used Pointer-generator Networks from \citet{pointernetwork} --- a hybrid approach that is uses an abstractive seq2seq model but with an explicit copy mechanism that can extract information from the source document.

\input{tables/cnndm_results_table}
\paragraph{Results} We show results in Table~\ref{tab:cnndm}. The more extractive approaches generally reach higher AIS subscores. This is a somewhat expected result --- extractive systems are less likely to output hallucinations as they are quoting information verbatim from the documents. As with Wizard of Wikipedia, the AIS scores of the gold reference summaries is surprisingly lower than the model output, which we will discuss more in Section~\ref{sec:goldref}.


\subsection{Table-to-Text ToTTo data}
\paragraph{Set-up} Lastly, we show the utility of extending AIS to a table-to-text task where $P$ is a table rather than a text document.  $S$ is a sentence generated by a model to describe some highlighted portion of the table.  We chose the ToTTo dataset \cite{parikh-etal-2020-totto}, testing with T5 and ByT5 models that were previously used with this data in the GEM benchmark \cite{gehrmann-etal-2021-gem}.  We experiment with two different sizes of ByT5 and three different sizes of the T5 architecture. As before, we sampled the output of 200 examples from the test set.  We also annotated 200 ground-truth references from examples in the dev. set (as the test set does not have gold-truth references publicly available).

\input{tables/totto_results_table}
\paragraph{Results} We show results in Table~\ref{tab:totto}. The model with the most ``interpretable'' responses was T5-base, with the ByT5 architectures being significantly less interpretable.  On the other hand, the T5 architecture responses were more likely to be flagged (according to the annotators this was because the flagged responses contained artefacts like unintelligible character encoding errors). Generally, we don't observe statistically significant differences in the AIS subscores though the larger architectures tended to have slightly lower AIS scores (similar to our observations of Table~\ref{tab:qrecc}).


==> AIS Paper (Arxiv Copy) - July 19, 2022/sections/human_eval.tex <==
\section{Human Evaluation Study}
\label{sec:human-study}
We evaluate the feasibility of human AIS assessment for three NLG tasks: conversational question answering, summarization, and table-to-text generation. To quantify the significance of human judgements, we present evaluators with the output of different models for each of the tasks.

The set-up for these annotation tasks is to ask annotators to rate the AIS quality of $s$, some model produced output given some attributed source $P$.  In the conversational QA and summarization settings, $P$ is a document or passage from a document, while in the table-to-text setting $P$ is a table and its description. For conversational QA, annotators are also provided with a context $c$, which is the set of previous conversation turns.  $c$ is used to help annotators understand the contextualized meaning of the model output, what we formally define as explicature in \S\ref{sec:explicatures}.

Because this is a challenging task with many possible edge cases (such as those discussed in Table~\ref{tab:implicit_examples}), we ask five annotators to judge each example.  In our results section, we compare to the consensus answer (if there is one) for simplicity.  In future work, researchers who wish to use AIS for evaluating systems might find use in distinguishing between cases that are more clear cut (i.e., unanimous) versus those where there may be some inherent ambiguity.

\subsection{Task Design}
\label{sec:task-design}
We break the annotation task into two stages described in \S\ref{sec:ann:int} and \S\ref{sec:ann:ais}, which mirrors the formal steps in the AIS definition (\S\ref{sec:ais-definition}) First, the annotators are asked if they are able to understand and identify the information being shared in the model output without seeing the source document (i.e., whether it is {\it interpretable} on its own).  Then, if the output is deemed interpretable, the annotators are shown the ``attributed source'' \textit{P} and asked whether all of the information that is shared in $S$ can be attributed to $P$ (i.e., whether it is {\it AIS}).  As described in the results sections, the splitting of the task into these two steps helps annotators to first filter out outputs that are badly formed (e.g., ungrammatical to the point of impeded intelligibility) or too ambiguous (e.g., unclear pronouns) to appropriately evaluate the attribution.  In the results, we report scores based on the annotator consensus (i.e., majority vote): the percent of total examples marked as interpretable ({\it Int} in Tables) and the percent of interpretable examples that were marked as AIS ({\it AIS}). In some datasets, certain examples were flagged as difficult to annotate due to legibility-related issues (see \S\ref{sec:ann:flag}).  For those cases, we separately report the percentage of examples that were flagged ({\it Flag}) and thus excluded from the interpretability and AIS scores.


\subsubsection{Interpretability Rating}
\label{sec:ann:int}
In the initial stage of the annotation task, we show the annotators the model output $s$ and any preceding context $c$ without showing the source. 
We ask them to identify the interpretability by posing a yes/no question. For example, in the summarization task the annotators are asked:

\emph{Is \textbf{all} of the information relayed by the system summary interpretable to you?}

Note that context $c$ is populated with preceding turns of the system--user interaction\footnote{Some interactions may contain no previous turns.} in the conversational QA task, whereas in summarization and table-to-text tasks it is always empty. In the instructions, the context $c$ is explicitly called out to be used in interpreting output $s$ in the conversational QA task.

Here, the goal is to tease out if the model-generated output $s$ contains any potential ambiguity that would prevent or misguide establishing attribution to its source $P$. Anaphora resolution is the main source of this type of ambiguity, where deictic elements do not have clear antecedents within $s$ or its context  --- for example, pronominal usage with an unclear or broken coreference chain or definite noun phrases as first mentions. Additionally, syntactic ambiguity or disfluency may also result in diminished interpretability of $s$ (see Examples E4, E5 in Figure~\ref{fig:explicatures}).

We acknowledge potential anthropomorphizing effects on how annotators interpret the system output \cite{gopnik1992child}. Because cooperative meaning co-construction between interlocutors is the default communicative strategy of inter-human interaction \cite{grice1975logic}, when faced with ambiguities and slight discrepancies in the system output, annotators may be ``forgiving'' of diminished interpretability, especially if the underlying source is present and can help recover missing context.

In our experiments we have found that not presenting the source at this stage is crucial for ensuring that evaluators are strict in their assessment of interpretability of the system output 
(see Figures~\ref{fig:AIS_QA_UI_1}, \ref{fig:AIS_Summ_UI_1}, and \ref{fig:AIS_T2T_UI_1} for how it was implemented in the task interface).

\subsubsection{AIS Rating}
\label{sec:ann:ais}
If an annotator selects ``yes'' for the interpretability question, we show them the source $P$ and ask them whether \textbf{all} of the information relayed in the output $s$ can be supported by $P$. For example, in the conversational QA task the annotators are asked:

\emph{Is \textbf{all} of the information provided by the system response {\it fully} supported by the source document?}

Note that the $P$ for the conversational QA task is the retrieved document that serves as the source of the system output $s$. In the summarization task $P$ is the original news article from which the summary in $s$ was derived. In the table-to-text task $P$ is the original table, highlighted cells, and table metadata (table title,  section title, and section text) from which the textual table description is generated.

In the instructions, we tell annotators to first think about all of the information that is contained the output including: what's directly stated in the output sentence verbatim as well as any explicatures that can be made from the output with respect to the context, such as inferring pronoun references from the conversational history.

Annotators are instructed to only mark output as attributable if it is clear that all parts can be directly inferred from the source. The instructions specifically call out to utilize the paraphrase test:

\emph{In determining this question, ask yourself whether it is accurate to say “the provided news article says\dots” or “according to the news article\dots” with the system summary following this phrase.}

If the output is misrepresenting information from the source because it is misleadingly worded, missing important context, or even changing only slight details, these cases are all counted as ``not fully attributable''.

\subsubsection{Flag Rating}
\label{sec:ann:flag}
A special rating is reserved for flagging items that would be disqualified from the the task altogether because they flout the range of possible relationships between the utterance, its context, and the source defined in \ref{sec:ais-definition}.

In practical terms, these are tasks that are too malformed for annotators to perform judgements on. This category includes tasks with rendering issues in the interface (missing task elements, e.g., empty utterance), corrupted text resulting in non-communicative utterances (bad text encoding, HTML artifacts), underspecified source (the source document itself is ambiguous because it is too short and may contain unresolved reference chains), or a source that is difficult to understand because it requires expert-level knowledge.

Once a task is flagged, it is disqualified from the rating queue of the annotator who flagged it. Other annotators may choose not to flag this item; cumulative ratings and interannotator agreements are calculated for all non-flagged ratings of a task (see the flag sections in the annotator guidelines for \href{sec:instructions_qa_flag}{conversational QA}, \href{sec:instructions_summ_flag}{summarization}, and \href{sec:instructions_t2t_flag}{table-to-text}) Section~\ref{sec:instructions_t2t_flag}.

\subsubsection{Limitations}
By asking yes/no questions, we can greatly reduce the complexity of this task for annotators.  However, for some applications of AIS measures, it may be useful to have more fine-grained measures.  Additionally, we ask annotators to evaluate the entire output (rather than sentences or specific spans) under the reasoning that if even one span within the model output is not AIS, then the whole output is not AIS (cf. \citet{maynez2020faithfulness}, \citet{durmus-etal-2020-feqa}).

We also acknowledge that there are other aspects of model output quality (e.g., relevance, non-redundancy, etc.) not evaluated here.  We focus on the separate evaluation of AIS as part of a focused effort towards quantifying the attribution itself, disentangled from other desirable generation qualities.

\subsection{Human Evaluation Procedure}
The ratings were performed by a group of nine paid full-time annotators under the guidance and supervision of a project manager. The annotator team is based in Hyderabad, India; the annotators are native speakers of the Indian dialect of the English language. The annotators do not have a background in linguistics. They were trained for this specific task.

Three separate user interfaces were developed for performing the evaluation in this study: one for the conversational QA tasks evaluating the output of models trained on QReCC and WoW datasets,  another for summarization tasks evaluating the output of models trained on the CNN/DM dataset and lastly one for table-to-text tasks evaluating the output of models trained on the ToTTo dataset. The interfaces share many fundamental design elements with task dependent modifications. For example, the conversation QA interface contains a devoted element for displaying the conversational history. All three interfaces explicitly hide the source document/table at the stage when interpretability of the system output is evaluated (see the Appendix for the interface layouts and annotator prompts (Figures~\ref{fig:AIS_QA_UI_1}, \ref{fig:AIS_QA_UI_2}, \ref{fig:AIS_Summ_UI_1}, \ref{fig:AIS_Summ_UI_2}, \ref{fig:AIS_T2T_UI_1}, and \ref{fig:AIS_T2T_UI_2}).

The annotators were trained on the tasks in a series of stages. First, a pilot study of 50--100 items was conducted with the first iteration of the annotator instructions. As part of the pilot, all ratings were required to have written justifications elaborating the reasoning for the provided rating. The results of the pilot were analyzed by the authors to identify common errors patterns; collected justifications were helpful in understanding the reasoning annotators used to arrive at their ratings. The results of the review were communicated back to the annotators, and the instructions were modified to emphasize areas leading to common ratings errors.

Next, a portion of the ratings was inspected by the authors for persistent error patterns and the feedback communicated to annotators. Additionally, the annotators collected edge cases where they found it difficult to make judgements. These edge cases were adjudicated by the authors; recurring complex patterns were used to expand the annotator guidelines (see the Appendix for full final instructions for \href{app:instructions_qa}{conversational QA}, \href{sec:instructions_summarization}{summarization}, and \href{sec:instructions_t2t}{table-to-text}).

Finally, the annotator team performed internal audits on a subset of completed tasks.

Annotators were initially trained on the conversational QA tasks; other tasks and training were introduced subsequently.


==> AIS Paper (Arxiv Copy) - July 19, 2022/sections/intro5.tex <==
\section{Introduction}\label{sec:intro}
Large, pretrained neural models have advanced Natural Language Generation (NLG) performance across a variety of use cases, including text summarization, translation, and dialogue.
Yet, generative neural models are  known to hallucinate often, lacking faithfulness to underlying sources, for example in summarization or in grounded dialogue systems. Accurate evaluation with respect to these issues is important.




In this paper, we develop a framework for the evaluation of {\em attribution}, by which we mean the accurate use of source documents to support generated text. Attribution is closely related to issues of hallucination and faithfulness (see \S\ref{sec:background} for discussion). As a key motivating example, consider a dialog with a system that generates responses to a user’s sequence of questions:

\begin{small}
\begin{tabbing}
\hspace{0.2cm} \= \textsc{User:} what was George Harrison’s first solo album?\\
\> \textsc{System:} \= it was “Wonderwall Music”, released in November 1968.\\
\> \textsc{User:} how old was he when it was released?\\
\> \textsc{System:} he was 25 years old
\end{tabbing}
\end{small}
\noindent

If such a system, in addition to generating responses, could attribute its statements to source documents, that is, provide sufficient and concise evidence for its claims, system designers and users alike could more readily ascertain the extent to which the information it provides is supported by underlying sources.
Prior work in NLG spanning diverse use cases such as summarization, dialogue response generation and data-to-text generation have investigated issues of faithfulness and  “hallucination”, but have not provided a uniform and formally expressed framework to measure these errors.  We discuss the relationship of our work to related work in \S\ref{sec:background}.

In \S\ref{sec:definitions}, we introduce our evaluation framework, Attributable to Identified Sources (AIS), that can be used to assess whether statements in natural language made by a system are derivable from a given underlying source. 
The definition of AIS (see \S\ref{sec:ais-definition}) formalizes the meaning of a sentence $s$ in context using the notion of explicatures~\cite{carston1988explicature,wilson2002relevance}\footnote{For example, in the above dialogue the explicature of “he was 25 years old” is “George Harrison was 25 years old when `Wonderwall Music' was released”: the latter explicature is evaluated for attribution. Note that this use of explicatures is closely related to prior work on decontextualization \cite{choi2021decontext}, see  \S\ref{sec:background} for more discussion.}, and defines attribution to some background information source $P$ in terms of an intuitive test, asking whether ``According to \textit{P}, \textit{s}''. 
It also accommodates system outputs whose meaning is uninterpretable.
AIS can be used as a pre-condition or in tandem with other metrics or evaluation frameworks to assess overall quality.
For example, characteristics of the underlying source (such as ``source quality''), the fluency of the generated text, and so forth, can be measured using complementary metrics that are out of scope in this work.

We propose specific instantiations of AIS for three NLG tasks (\S\ref{sec:human-study}): 
response generation in a conversational QA setting (as in the example above; responses must be attributable to a provided answer document),
text summarization (where the summary must be attributable to the source article), and description generation from structured tables, or table-to-text (where the description must be attributable to the source table and associated metadata).
Each domain involves a number of challenges: for example, in dialogue systems a key challenge is that the meaning of system responses is highly contextually dependent.

Next, we establish the feasibility of AIS evaluations via an empirical study through conducting human evaluation experiments.
We train annotators to evaluate output text from multiple models per task using task-specific instantiations of AIS.
We show that in our human evaluation studies, it is possible to achieve a moderate to high degree of inter-annotator agreement (see \S\ref{sec:human-study} for more details).  We're also able to observe differences in model outputs' AIS scores, following generally expected trends.
As part of this work, we release the detailed guidelines for human evaluation.
We believe that AIS as a framework would be essential for the evaluation of system-generated utterances across NLG tasks.

==> AIS Paper (Arxiv Copy) - July 19, 2022/sections/linguistic3.tex <==
\section{A Formal Definition of Attributable to Identified Sources}
\label{sec:definitions}

This section gives a formal definition of AIS, attempting to give a clear and precise definition of attribution. We  first  give  a  definition  of  AIS  for  a  simple case, where the utterance from a system is a standalone proposition.  In spite of the simplicity of this  setting,  it  is  highly  informative,  and  forms the  basis  for  the  full  definition  of  AIS. We then describe  how  this  definition extends to a much larger set of system utterances, in particular giving a treatment of \emph{interpretability}\footnote{We acknowledge that the term "interpretability" has come to signify "model interpretability" in the NLP and ML community (as established in \citet{harrington1985harvey}, \citet{ribeiro2016model}). The term in our use represents how interpretable system output is for a human annotator. The choice of terminology is intended to be more conceptually transparent when used by annotators: unlike other terms like "meaningful"/"nonsensical" \cite{durmus-etal-2020-feqa}, or "sensibleness"~\cite{adiwardana2020towards}, "interpretability" more readily alludes to the significance of the propositions in system generated output in relationship to context. Finally, the annotators are typically not familiar with the "model interpretability" usage of the term.}, and \emph{contextual effects}. A key idea in our model of meaning in context is the notion of explicatures~\cite{carston1988explicature,wilson2002relevance,choi2021decontext}. In a final subsection, we describe how key aspects of the AIS definition naturally lend it to operationalization, while also pointing out how certain idealizations (e.g., the notion of a ``generic speaker”) must be relaxed to accommodate the practical realities of implementation.

\subsection{An Initial Definition of AIS: Attribution of Standalone Propositions}

We now give a definition of AIS for a simple but important case, where the text in question is a {\em standalone proposition}. We in general assume a setting where AIS is to be determined for a string whose meaning is ascertained relative to a context. In the following treatment we assume that time is the only non-linguistic aspect of context relevant to determining textual meaning, modeling a setting where two generic speakers communicate over a text-based channel, with no additional prior information about each other.\footnote{Extensions of AIS to more complex settings may require a more elaborate notion of non-linguistic context.}

We define standalone propositions as follows:

\begin{definition}[Standalone Propositions]
A standalone proposition is a declarative sentence that is interpretable once a time $t$ has been specified.
\end{definition}
\noindent 
To illustrate the definition of standalone propositions, consider the following examples:
\begin{description}
\item[Example S1:] George Harrison was 25 years old when his album `Wonderwall Music' was released.

\item[Example S2:] He was 25 years old.

\item[Example S3:] George Harrison was 25 years old.

\item[Example S4:] George Harrison died over 15 years ago.
\end{description}

\noindent 
All four examples are declarative sentences. S1 is a standalone proposition. S4 is a standalone proposition, as it is interpretable once the time $t$ is specified. 
S2 is however not a standalone proposition, as it cannot be interpreted without additional contextual information: It is unclear what "He" refers to.
More subtly, S3 is also not a standalone proposition, because it lacks details of historical context.

The definition of AIS for standalone propositions is as follows:

\begin{definition}[AIS for standalone propositions]
A pair $(s, t)$ consisting of a standalone proposition $s$ and a time $t$ is Attributable to Identified Sources (AIS) iff the following conditions hold:
\begin{enumerate}
    \item The system provides a set of parts $P$ of some underlying corpus $K$, along with $s$.
    \item $(s, t)$ is attributable to $P$. 
\end{enumerate}

\noindent
A pair $(s, t)$ is {\bf attributable} to  a set of parts $P$ of some underlying corpus $K$ iff:
A generic hearer will, with a chosen level of confidence, affirm the following statement:
 “According to $P$, $s$'', where $s$ is interpreted relative to time $t$.
\end{definition}

\noindent 
Here, the corpus $K$ could be a set of web pages, and the parts $P$ could be pointers to paragraphs or sentences within $K$; or the corpus $K$ could be a knowledge graph, with $P$ as parts of the underlying knowledge graph; other examples are no doubt possible. 

As an example, consider standalone proposition S1 given above, assume that the corpus $K$ is all of Wikipedia, $t_0$ is the present time (specifically, noon on December 21st 2021), and assume that the set $P$ consists of a single paragraph from Wikipedia, as follows:

\begin{description}
\item[Example P1:] George Harrison (25 February 1943 --- 29 November 2001) was an English musician, singer--songwriter, and music and film producer who achieved international fame as the lead guitarist of the Beatles. His debut solo album was
`Wonderwall Music', released in November 1968.
\end{description}
\noindent 
Under this definition, it would be correct for a hearer to judge ``$(S1, t_0)$ is attributable to P1'', because the ``according to'' test in the AIS definition holds. That is, it is reasonable to say according to P1, S1'' where S1 is interpreted at time $t_0$: ``according to P1, George Harrison was 25 years old when his album `Wonderwall Music' was released.''

Note that in some cases the system may provide multiple parts. The standalone proposition $S$ may also be justified by certain forms of multi-hop reasoning (e.g., arithmetic processes) over that set of parts. The above example requires reasoning about dates and age.

\input{tables/madeupexamples}


\subsection{Extending AIS: Attribution of Sentences in Context}
We now extend the previous definition of AIS to cover sentences that that go beyond standalone propositions. To do so, we will need to consider multi-sentence cases, and cases with non-empty linguistic contexts. We will also cover cases that are uninterpretable. 

We first define the notion of ``utterance'':
\begin{definition}[Utterance]
An utterance is a sequence of one or more {\em sentences} produced by a system or user, where a sentence may be a declarative, a question, a command, an exclamation, or a fragment. The $i$th system utterance is  $s_i = s_{i,1} \ldots s_{i, |s_i|}$, where $s_{i,j}$ is the $j$th sentence within system utterance $s_i$, and similarly the $i$th user utterance is $u_i = u_{i,1} \ldots u_{i, |u_i|}$.
\end{definition}

To briefly illustrate our approach to non-empty linguistic contexts, consider the following interaction between a user and system (originally given in the introduction; repeated here for convenience):

\begin{small}
\begin{tabbing}
\hspace{0.2cm} \= $u_1$: what was George Harrison’s first solo album?\\
\> $s_1$: \= it was “Wonderwall Music”, released in November 1968.\\
\> $u_2$: how old was he when it was released?\\
\> $s_2$: he was 25 years old.
\end{tabbing}
\end{small}

\noindent
The system utterance $s_2 = \hbox{\em he was 25 years old}$ is clearly not a standalone proposition. As such, it cannot be evaluated for AIS given our previous definition. However, given the previous context in the interaction, intuitively the meaning of $s_2$ is something similar to the standalone proposition ``George Harrison was 25 years old when his album ``Wonderwall Music'' was released''. This latter ``paraphrase'' of $s_2$'s meaning is a standalone proposition, and can be evaluated using the AIS definition for standalone propositions.

We will make this notion of ``paraphrase'' of the meaning of an utterance in context more formal, through the introduction of {\em explicatures}. The explicature of $s_2$ in context of the previous utterances $u_1, s_1, u_2$ is $e$ = {\em George Harrison was 25 years old when his album ``Wonderwall Music'' was released}. Once explicatures have been defined in this way, they can be evaluated for AIS in exactly the same way as standalone propositions.

\subsubsection{Definition of Interactions and Linguistic Context}

We will use the following definition of {\em interaction} throughout the paper:
\begin{definition}[Interactions]
An {\em interaction}  consists of: 1) a sequence $u_1 \ldots u_m$ of $m \geq 0$ user utterances; 2) a sequence $s_1 \ldots s_n$ of $n \geq 0$ system utterances; 3) a strict total order over the $m + n$ user and system utterances.\footnote{For example, the order might be specified by functions $U: \{1 \ldots m\} \rightarrow \{1 \ldots (m + n)\}$ and $S: \{1 \ldots n\} \ldots (m+n)\}$ where $U(i)$ (respectively $S(i)$) is the position of utterance $u_i$ (respectively $s_i$) in the total ordering. The notational details will not be important for this paper.
}
\end{definition}

\noindent 
This setting is intended to be quite general, including a broad class of applications where systems generate utterances. In conversational QA systems we typically have alternating user and system utterances, where $m = n$, and the total ordering is $u_1, s_1, u_2, s_2, \ldots u_n, s_n$. In summarization tasks we have a simplified setting where $m = 0$, $n = 1$, and $s_1$ is equal to the summary generated by the system. Table-to-text tasks are similar to summarization in that $m = 0$, $n = 1$, while $s_1$ is the description of the table generated by the system.

Each sentence has an associated linguistic context:

\begin{definition}[Linguistic Context for Sentences]
We define the linguistic context for system sentence $s_{i,j}$ to be $c_{i,j}$, where $c_{i,j}$ is the ordered sequence of sentences (with speaker identities, user or system) that precedes $s_{i,j}$ in the total ordering. 
We define the linguistic context for user sentence $u_{i,j}$ to be $c'_{i,j}$, where $c'$ is defined in a similar way.\footnote{An equally plausible definition would be to define $c_{i,j}$ to also include the following sentences within utterance $s_i$, that is, $s_{i,j-1}, s_{i,j+1} \ldots s_{i, |s_i|}$ (and an analogous definition for $c'_{i,j}$). That is, the context would be extended to include sentences that follow $s_{i,j}$ in the utterance $s_{i}$. This would allow instances of cataphora, for example, to be handled in the definitions of explicatures and attribution.}
\end{definition}


\noindent 
Here the definition of "sentence" is intended to be quite broad. A sentence could be a declarative sentence, a question, or a fragment (such as the string "25 years old"). Under the above definitions, the context for a user or system sentence is
simply the sequence of user and system sentences that precedes it. To illustrate these definitions consider the following example:

\begin{small}
\begin{tabbing}
\hspace{0.2cm} \= $u_1$: what was George Harrison’s first solo album?\\
\> $s_1$: \= it was “Wonderwall Music”, released in November 1968.\\
\> $u_2$: how old was he when it was released?\\
\> $s_2$: He was 25 years old. It was the first solo album by a member of the beatles.
\end{tabbing}
\end{small}

\noindent
Here the system utterance $s_2$ consists of two sentences, $s_{2,1} =$ {\em He was 25 years old} and $s_{2,2} =$ {\em It was the first solo album by a member of the Beatles}.




\subsection{Explicatures}\label{sec:explicatures}

A key goal in this section is to define AIS for sentences $s_{i,j}$ in linguistic contexts $c_{i,j}$ which are non-empty (i.e., which contain previous sentences in the discourse). To do this it will be critical to formalize what is meant intuitively by "the meaning of $s_{i, j}$ in context $c_{i, j}$". To do this we introduce {\em explicatures} (this definition is closely related to definition 1 in \citet{choi2021decontext}):

\begin{definition}[Explicatures]
Define the context $c$ to be $(c_l, t)$, where $c_l$ is the linguistic context and $t$ is the time. Define  $\bar{c}$ to be the context $(\epsilon, t)$ where $\epsilon$ is the linguistically empty context: that is, $\bar{c}$ is a copy of $c$ but with $c_l$ replaced by $\epsilon$.
The set of {\em explicatures} $E(c, x)$ of a sentence $x$ in a context $c$ is a set  that satisfies the following conditions: 1) each $e \in E(c, x)$ is a declarative sentence or question that is interpretable in context $\bar{c}$; 2) each $e \in E(c, x)$ has the same truth-conditional meaning in $\bar{c}$ as the meaning of sentence $x$ in context $c$. 
\end{definition}
\noindent 
Note that the sentence $x$ will most often in this paper be a system sentence $s_{i, j}$ in linguistic context $c_{i,j}$, but can also be a user sentence $u_{i, j}$ in linguistic context $c'_{i,j}$.

Thus, each $e \in E(c, x)$ is a paraphrase of $x$ that is interpretable in the linguistically empty context and that preserves the truth-conditional meaning of $x$ in context $c$. Note that $E(c, x)$ is a set because there may be multiple ways of paraphrasing $x$, which are equivalent in meaning. Given an equivalence relation between sentences that identifies whether any two sentences are equal in meaning or not, we can think of a single member of $E(c, x)$ as a representative of the entire set $E(c, x)$. Following this, in a slight abuse of terminology we will henceforth often write "the explicature of $x$ in context $c$ is $e$" as if there is a single unique explicature $e$, with the understanding that $e$ represents the entire set $E(c, x)$. We will also write $E(c, x) = e$ as shorthand for $E(c, x)$ being equal to the set of all sentences whose meaning is the same as that of $e$.

In addition, we define interpretability as follows:
\begin{definition}[Interpretability]
A sentence $x$ in context $c$ is {\em uninterpretable} if the truth-conditional meaning of $x$ in context $c$ is unclear. In this case we write $E(c, x) = \enull$.
\end{definition}

Figure~\ref{fig:explicatures} shows several examples illustrating these definitions. Some key points are as follows:

\hspace{1ex}

\noindent
{\em Remark 1:}
    In example E1, the system response is a direct answer to a question, $s_{2,1} = $ {\em 25 years old}. $s_{2, 1}$ itself is not a declarative sentence, but given the context (in particular the question it is answering), its explicature is the standalone proposition {\em George Harrison was 25 years old when "Wonderwall Music" was released}. This type of example --- where a direct answer to a question is an entity, noun-phrase, or some other fragment, but its explicature is a standalone proposition --- is important and frequent. As another example consider the following:
    
\begin{tabbing}
\hspace{0.2cm} \= $u_1$: What was George Harrison’s first solo album?\\
\> $s_1$: Wonderwall Music\\
\>$E(c_{1,1}, s_{1,1}) = $ \= {\em George Harrison's first solo album em was "Wonderwall Music"}
\end{tabbing}

\noindent
{\em Remark 2:} In Example E3, the system segment is a sequence of two declarative sentences. Each sentence has an explicature that is a standalone proposition. This type of case is again frequent and important.

\hspace{1ex}

\noindent
{\em Remark 3:} In Example E4 the system utterance is uninterpretable, because it is not clear what "the band" is referring to. Example E5 contains disfluencies that make it difficult to reliably interpret: "it" is not the expected pronominal reference; in this context "25" becomes too ambiguous to interpret as referring to the age of a human entity. 

\hspace{1ex}

\noindent
{\em Remark 4:} Examples E6 and E7 contain questions in the system and user utterance respectively. These examples illustrate that single questions (E7) or questions within multi-sentence utterances (E6) have well-defined explicatures. 


\begin{figure}[!t]
\begin{small}
\begin{tabbing}
{\bf Example E1}\\
\hspace{0.2cm} \= $u_1$: what was George Harrison’s first solo album?\\
\> $s_1$: it was “Wonderwall Music”, released in July 2006.\\
\> $u_2$: how old was he when it was released?\\
\> $s_2$: 25 years old\\
\> $E(c_{2,1}, s_{2,1})$ = \= {\em George Harrison was 25 years old when "Wonderwall Music" was released}
\end{tabbing}

\begin{tabbing}
{\bf Example E2}\\
\hspace{0.2cm} \= $u_1, s_1, u_2$ as in Example E1\\
\> $s_2$: he was 25 years old\\
\> $E(c_{2,1}, s_{2,1})$ = \= {\em George Harrison was 25 years old \em when "Wonderwall Music" was released}
\end{tabbing}

\begin{tabbing}
{\bf Example E3}\\
\hspace{0.2cm} \= $u_1, s_1, u_2$ as in Example E1\\
\> \=$s_2$: He was 25 years old. It was the first solo \\
\> \> album by a member of the Beatles.\\
\> $E(c_{2,2}, s_{2,2})$ = \=  {\em Wonderwall Music was the first solo album by a member of the Beatles.}
\end{tabbing}

\begin{tabbing}
{\bf Example E4}\\
\hspace{0.2cm} \= $u_1, s_1, u_2$ as in Example E1\\
\> $s_2$: the band was The Beatles\\
\> $E(c_{2,2}, s_{2,2})$ = \= $\enull$
\end{tabbing}

\begin{tabbing}
{\bf Example E5}\\
\hspace{0.2cm} \= $u_1, s_1, u_2$ as in Example E1\\
\> $s_2$: it was 25\\
\> $E(c_{2,2}, s_{2,2})$ = \= $\enull$
\end{tabbing}

\begin{tabbing}
{\bf Example E6}\\
\hspace{0.2cm} \= $u_1, s_1, u_2$ as in Example E1\\
\> \=$s_2$: He was 25 years old. Have you heard that album? \\
\> $E(c_{2,2}, s_{2,2})$ = \= {\em Have you heard the album "Wonderwall Music"?}
\end{tabbing}

\begin{tabbing}
{\bf Example E7}\\
\hspace{0.2cm} \= $u_1$: what was George Harrison’s first solo album?\\
\> $s_1$: it was “Wonderwall Music”, released in July 2006.\\
\> $u_2$: how old was he when it was released?\\
\> $E(c'_2, u_2)$ = \= {\em how old was George Harrison when "Wonderwall Music" was released?}
\end{tabbing}

\end{small}
\caption{Examples of utterances in context, and their explicatures.}
\label{fig:explicatures}
\end{figure}

\label{sec:ais}

\subsubsection{The Full Definition of AIS}
\label{sec:ais-definition}

With this background, we can now give the full definition of AIS:

\begin{definition}[AIS, full definition]
\label{defn:ais-full}
A pair $(s, c)$, where $s$ is a sentence and $c=(c_{l}, t)$ is a pair consisting of a linguistic context and a time, is {Attributable to Identified Sources (AIS)} iff the following conditions hold:
\begin{enumerate}
    \item The system provides a set of parts $P$ of some underlying corpus $K$, along with $s$.
    \item $s$ in the context $c$ is interpretable (i.e., $E(c, s) \neq \enull$).
    \item The explicature $E(c, s)$ is a standalone proposition.
    \item The pair $(E(c, s), t)$ is attributable to $P$. 
\end{enumerate}

\noindent
The pair $(E(c, s), t)$ is {\bf attributable} to  a set of parts $P$ of some underlying corpus $K$ iff:
A generic hearer will, with a chosen level of confidence, affirm the following statement:
 “According to $P$, $E(c, s)$”, where $E(c, s)$ is interpreted relative to time $t$.
\end{definition}
\noindent 
The definition is very similar to the earlier definition of AIS for standalone propositions, but with checks for interpretability, and with attribution applied to explicatures of system sentences. Note that AIS can only hold for system sentences that have an explicature that is a standalone proposition  (condition 3). For example, the explicature in Example E6 in Figure~\ref{fig:explicatures} is not a standalone proposition, as it is a question. We leave the treatment of cases such as these to future work (we might for example evaluate attribution for declarative sentences within the explicature, excluding questions; or we might evaluate presuppositions within the questions themselves).

\subsubsection{Attribution of Entire Utterances}

In the previous sections we have described AIS for the individual sentences $s_{i,1} \ldots s_{i,|s_i|}$ within a system utterance $s_i$. This assumes that such a segmentation of the utterance into sentences is available, for example, it is provided by the system. An alternative is to evaluate entire utterances $s_i$ for AIS, in a "single-shot" annotation. AIS applied at the utterance level could potentially have the advantages of simplicity, and the avoidance of segmenting utterances into sentence boundaries. It has the potential disadvantage of being coarser grained, not allowing AIS judgments at the sentence level. The choice of sentence-level vs. utterance-level AIS will depend on the exact application of AIS.

It should be relatively straightforward to extend the full definition of AIS (Section~\ref{sec:ais-definition}) to apply to multi-sentence utterances. The definition of explicatures would need to be extended to multi-sentence utterances; the definition of standalone propositions would also have to be extended to apply to multiple sentences; the definition of "attributable" would also need to be extended.


\subsection{Towards Operationalization of AIS}
\label{sec:operationalization}
In the above definition of AIS, three definitions are of key importance: 1) the     ``according to'' test for standalone propositions; 2) the definition of interpretability; 3) the definition of explicatures, which are related to the interpretation of utterances in non-empty linguistic contexts. 
Note that it is not necessary for annotators to explicitly wield all of these definitions, or come to understand any of them in entirely formal terms, in order to provide AIS judgments. 
In developing human annotation guidelines for annotators who do not necessarily have background in these concepts, we relay the ``according to'' test and interpretability in a way that leverages natural speaker intuitions. We convey explicature through the more intuitive idea of a sentence paraphrase with respect to linguistic context.
Annotators are instructed to apply the ``according to'' test strictly, without making further assumptions beyond what is conveyed in the text. 

The formal definition of AIS makes several idealizing assumptions that must be relaxed in practical settings. 
In lieu of the posited ``generic hearer'', the judgments of actual annotators will naturally be influenced by the particulars of their interpretive capacities, stemming from differences, for example, in cultural background and domain expertise.
Table~\ref{tab:implicit_examples} lists several instances where such differences could conceivably affect judgments.
These effects are, to some extent, inherent to implementing AIS using human judgments.

==> AIS Paper (Arxiv Copy) - July 19, 2022/sections/quality.tex <==
\subsection{Annotation Quality}
In this section we discuss the further implications of the human annotation results.  We focus on two primary questions: (1) can humans reliably annotate AIS? and (2) what do our measured AIS ratings indicate about NLP data and models?

\subsubsection{Interannotator Agreement}
\input{tables/iaa}
We show the interannotator agreement (IAA) for crowd annotators in the left half of Table~\ref{tab:iaa}.  The metrics we used include Krippendorff's alpha comparing individual ratings, pairwise agreement (PA) comparing individual ratings and an F1 score comparing individual ratings to the consensus (majority vote). Agreement results are generally moderate to high, displaying that --- while this is a challenging task --- the annotators are able to be fairly consistent with one another.  The alpha scores are generally lowest on the summarization CNN/DM task, perhaps because the output text is much longer in summarization, increasing the complexity of the rating task.  The F1 scores are similarly high, particularly on the AIS ratings.

\subsubsection{Audits}
\input{tables/qc_stats}
Separately, the annotator team also performed  internal audits on the annotation quality where a project lead from the annotator team examined a sample of individual annotator judgements at different points (snapshots) of the annotation process (Table~\ref{tab:qc_stats}). QRECC and WoW annotations were evaluated together as the broader conversational QA annotation task. The overall reported quality is in the high nineties for all three tasks with slight variations. The annotation quality for the conversational QA tasks remains high across all snapshots; we attribute this to the annotators extended experience with the task prior to the annotation of this dataset\footnote{The annotator pool was involved in annotating a series of related tasks for Conversational QA beyond the reported results in this paper.}. The quality of the summarization annotations shows an increase over snapshots, as annotators internalize the guidelines and gain expertise in the task. The quality of the table-to-text annotations fluctuates and is generally the lowest of the three tasks; we attribute this to a much larger sample for which quality was measured. Overall, across the three tasks, the larger the quality evaluated sample, the lower the overall reported quality. Barring genuine task differences that would lead to variations in annotation quality, this suggests that the reported table-to-text quality of annotations is the most representative of all three tasks. 

\subsubsection{Crowd Annotator Performance}
\input{tables/completion_time_table}
We also observe average task completion times decrease across all types of tasks as the annotators are exposed to more tasks and internalize the instructions (Table~\ref{tab:completion_time}). Initial pilots for the conversational QA, summarization, and table-to-text tasks included required rating justifications for interpretability and AIS questions as part of annotator training. Once the production annotation started and the justifications were no longer required, completion times decreased significantly for all types of tasks, which we attribute primarily to the annotators no longer typing out detailed justifications of their ratings, but also overall internalization of the guidelines. The effects of annotators internalizing the guidelines are also evident when comparing completion times at production annotation start and finish: average task completion times decrease for all three types of tasks as annotators are exposed to more tasks and gain more experience.

At the same time, the absolute task completion times are consistently and substantially different across the three tasks suggesting their uneven complexity, with conversational QA taking the shortest amount of time to complete, summarization requiring the longest, and table-to-text falling in-between. This pattern follows the trend in the distribution of inter-annotator agreement across the three tasks: tasks with shorter completion times generally have higher interannotator agreement. We postulate that this is primarily due to the difference in the amount of context that is necessary to perform ratings. Although conversational QA tasks may contain several turns of preceding interactions between the system and the user as well as the source document, the amount of information in the source articles in the summarization task is substantially larger. Likewise, source tables in the table-to-text task can be extensive and have the added information complexity of cell highlighting and table metadata. Finally, register and discourse structure effects may be at play here as well. Conversational QA tasks build upon colloquial interactions between the user and the system, setting up the context of the interaction in shorter utterances and helping annotators anticipate the contents of the source document. Likewise, Wikipedia, news articles, and tables package information differently as they serve somewhat different communicative goals, and it is possible that one of these source types is more amenable to inspection required for performing AIS ratings. 

\subsubsection{Expert Ratings}
\input{tables/examples_conv_expert}
\input{tables/examples_summ_expert}
Where AIS is used as a metric for ranking generative models, the internal consistency of crowd annotations is paramount. But, to help illuminate the inherent challenges in calibrating this annotation task, we also compare the crowd ratings with those of expert on a small set of examples.
Due to the challenges of scaling expert evaluations, we limited expert ratings to two tasks (CNN/DM and QReCC) with 50 examples each.  The experts (two co-authors) first annotated the examples separately from each other using the same interface as the crowd annotators and then discussed their answers to reach a consensus. \emph{Expertise} here might be derived from general educational background (a different approach to close reading), the ability to discuss annotations (and to do so carefully at self-guided pace), specialized knowledge, and first-hand familiarity with the evaluation framework. Expertise does not imply that the experts have more experience performing the task than the crowd annotators.

In order to account for natural ambiguity in assigning a rating category, experts marked some cases as ``either option acceptable''. We compare the individual crowd annotator ratings to the expert consensus in the right half of Table~\ref{tab:iaa}. Crowd annotators tend to agree with each other more than they agree with experts, which is expected due to differences in background, incentives, and procedure, although there is still reasonably consistent agreement in most cases.  On closer inspection, we find that most disagreements are cases where there is underlying ambiguity caused by vagueness in the evidence or model output. In these cases experts erred more on the side of being critical of the model and crowd annotators erred more towards being lenient.  In the case of conversational QA, most of the AIS disagreements involved cases where the document and the response do not refer to an entity using the same naming conventions (e.g., using both first and last name; see Table~\ref{tab:examples:qa:exp}) leaving some ambiguity that the document is referring to the same entity as the response. The greatest source of disagreements overall is the interpretability question in the summarization task (see examples in Table~\ref{tab:examples:summ:int}).  The summaries in the CNN/DM dataset were originally crawled from high-level article highlights, and experts observed that --- due to the linguistic style of these highlights --- there were many cases where the language may be vague or ambiguous, making this dimension more challenging. 
Because we use interpretability as a pre-filtering stage for the AIS question, we make allowances for the annotators being more inclusive.  Despite the differences on the interpretability dimension, they generally agreed with experts on most AIS questions, our primary evaluation dimension.

\input{tables/examples_reference}
\subsubsection{Limitations of Gold References}
\label{sec:goldref}
The last rows in Tables \ref{tab:qrecc}, \ref{tab:wow}, \ref{tab:cnndm} and  \ref{tab:totto} show annotation results on reference answers sampled from these datasets.  The results demonstrate that there is actually a limit on the AIS quality of the data itself in multiple tasks.  We include examples of non-AIS references in Table~\ref{tab:examples:notais:ref} to illustrate what some of these examples look like.  We hypothesize that this is because the originators of the data were not specifically instructed to be as faithful to the underlying documents as possible.  In the case of Wizard of Wikipedia \citep{dinan2019wizard}, the gold response is only AIS 16\% of the time.  But, this dataset was constructed for a different objective --- to contain \emph{both} informative and engaging responses. The MTurk workers who created the data were provided documents to enhance their conversations but could do so at their own discretion, often including their own thoughts and opinions in the conversation as well. This is also reflected in the CNN/DM AIS scores --- summaries in CNN/DM are only attributable to the documents in 54\% of the interpretable examples. 
Looking more closely, we speculate that this may be due to the post-hoc data creation process used to extract summaries from article highlights written by journalists.  We observed that the reference summaries in CNN/DM may sometimes refer to external pieces of information that may have accompanied the article (a picture, a headline, etc.) or sometimes make assumptions about what the intended audience of the article might already know that can affect either the interpretability or AIS scores (see Example 1 in Table~\ref{tab:examples:notais:ref} and Example 3 in Table~\ref{tab:examples:notint}). These results indicate that there is still a need for high-quality AIS data for training new NLG models.

\subsubsection{Examples}
In the Appendix, we separately list textual examples rated as uninterpretable (Table~\ref{tab:examples:notint}), interpretable but not AIS  (Table~\ref{tab:examples:notais}), or both interpretable and AIS (Table~\ref{tab:examples:ais}).  For the table-to-text task, we present examples in a more visual figure,  Figure~\ref{fig:ttt:ex}, for better legibility.  Common factors in marking text as ``uninterpretable'' include repetitive, degenerate language and ambiguous pronouns and ellipses.  Additionally, some outputs are marked as uninterpretable because they are hard to understand ``on their own''.  Whether or not a piece of text can be understood may also rely on things like commonsense and background knowledge that could vary depending on annotators' backgrounds (see Example 3 from Table~\ref{tab:examples:notint}). Ambiguous references can also affect both interpretability and the AIS scores.  In Example 2 of Table~\ref{tab:examples:notais}, the retrieved document did not provide enough information to completely verify the response since it never refers to Ann Veneman by her full name.  This is a seemingly minor detail, but annotators were often sensitive to this type of example since they could not verify whether the document was actually referring to the same entity as the model output.  Another type of non-AIS output that frequently appeared in the QReCC data were cases where a model outputted a seemingly informative statement that --- instead of being grounded to the document --- was actually grounded to a previous conversation turn, sometimes repeating itself verbatim.
Lastly, examples verify that AIS evaluations can be disentangled from other quality aspects, such as conversational relevance. This was challenging to instruct to annotators as it is instinctual to judge quality more holistically, and they were explicitly given instructions with multiple examples illustrating what types of quality aspects to ignore. In the resulting annotations, they would mark incoherent summaries or irrelevant conversational replies as AIS if they conveyed well supported information, appropriately disregarding other aspects of quality.


==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/cnndm_results_table.tex <==
\begin{table*}
    \caption{Results of human study on 200 examples from CNN/DM test set (randomly sampled).  Of the three models we tested with, unsurprisingly the more extractive models have higher AIS scores. }
    \begin{tabularx}{\textwidth}{l|l|ll}
    \toprule
        Model & Approach & Int & AIS  \\
        \midrule
        MatchSum \cite{matchsum} & Extractive &90.0 & 99.4\\
        Pointer-Gen \cite{pointernetwork} & Hybrid & 90.0 & 97.8\\
        BigBird \cite{bigbird} & Abstractive & 90.0 & 87.2$^*$ \\
        \midrule
        {\it Reference} &-& 86.0 & 54.1$^*$ \\
    \bottomrule
    \end{tabularx} \\
    \tabnote{\footnotesize{* Indicates that the result is significantly lower than the \textbf{highest score} in the column (with $p<0.01$).}}
    \label{tab:cnndm}
\end{table*}



==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/completion_time_table.tex <==
\begin{table*}[th]
    \caption{Average completion times (\textit{ACT}) for ratings tasks in seconds. Conversational QA tasks include evaluation of generated text for QReCC and WoW. Summraziation tasks include evaluation of generated text for CNN/DM. Table-to-text tasks include evaluation of generated text for ToTTo. Justifications were required for all question tasks at the pilot stage, but not at the production stages. Average completion times decrease for all three task types as annotators gain more experiences over the amount of observed tasks (\textit{Tasks}), but are always relatively longer for summarization. Note that the average completion times may be reduced further for summarization with more tasks observed by annotators, a pattern we see in the conversational QA and table-to-text task types.}
    \begin{tabularx}{\textwidth}{l|l|lX|lX|lX}
    \toprule
    & &\multicolumn{2}{c|}{Conversational QA}
    &\multicolumn{2}{c|}{Summarization}
    &\multicolumn{2}{c}{Table-to-Text}\\
        Stage & Justification & Tasks & ACT, secs. & Tasks & ACT, secs. & Tasks & ACT, secs. \\
        \midrule
        Pilot & $+$ & 75 & 375.30 & 50 & 687.02 & 100 & 324.72 \\
        Start & $-$ & 762 & 136.76 & 187 & 308.14 & 136 & 238.40 \\
        Finish & $-$ & 4,022 & 73.19 & 900 & 263.55 & 1,496 & 193.95 \\
    \bottomrule
    \end{tabularx}
    \label{tab:completion_time}
\end{table*}

==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/iaa.tex <==
\begin{table*}
    \caption{Annotator agreement measured as interannotator agreement (left half of the table) or as agreement with expert consensus (right half of the table, only measured on QRECC and CNN/DM tasks).  Metrics include --- F1: a F1 measure comparing individual ratings to the consensus rating; PA: pairwise agreement as percentage of individual pairs that agree; $\alpha$: Krippendorff's alpha measure comparing pairs of individual ratings.}
    \begin{tabular*}{\textwidth}{l|lll|lll|lll|lll}
    \toprule
       & \multicolumn{6}{c}{IAA} & \multicolumn{6}{c}{vs. Expert} \\
       & \multicolumn{3}{c}{Int} & \multicolumn{3}{c}{AIS} & \multicolumn{3}{c}{Int} & \multicolumn{3}{c}{AIS} \\
        Task &  F1 & PA & $\alpha$&  F1 & PA & $\alpha$&  F1 & PA & $\alpha$&  F1 & PA & $\alpha$  \\
        \midrule
        CNN/DM & .83&.80&.46&.92&.89&.69&.48&.60&-.04&.81&.86&.61 \\
        QReCC & .97&.96&.91&.93&.89&.76&.77&.81&.54&.77&.78&.54\\
        WoW & .88&.93&.60&.95&.88&.79 &-&-&-&-&-&-\\
        ToTTo & .95 &.95&.84&.92&.92&.74 &-&-&-&-&-&-\\
    \bottomrule
    \end{tabular*}
    \label{tab:iaa}
\end{table*}

==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/madeupexamples.tex <==
\begin{table*}
    \small
    \caption{AIS examples illustrating challenges in AIS judgements. These types of examples may be difficult to assess for AIS because they need extra reasoning, or assumptions about shared knowledge.  These examples are purely illustrative (not from real data examples).}
    \begin{tabularx}{\textwidth}{X X X}
    \toprule
    Evidence & Proposition Candidate & Challenges\\ 
    \midrule
George   Harrison   (25   February 1943  —  29 November 2001) was  an  English musician\dots  His debut solo album was `Wonderwall Music’, released in November 1968. & George Harrison was 25 years old when his album 'Wonderwall Music' was released. & \textit{Common sense and cultural knowledge is required to interpret the information in the proposition as it requires inferring that ``his'' is still referring to George Harrison. "George" is typically a male name in English; musicians release albums; therefore, "his album" likely refers to George Harrison, but not another unattested entity.} \\
    \midrule
The runtime of the theatrical edition of ``The Fellowship of the Ring'' is 178 minutes, the runtime of ``The Two Towers'' is 179 minutes, and the runtime of ``The Return of the King'' is 201 minutes. & The full run-time of ``The Lord of the Rings'' trilogy is 558 minutes. & \textit{Evaluating this requires numerical reasoning, and it also requires knowing that ``The Lord of the Rings'' trilogy consists of the three films mentioned (background knowledge that may vary from person to person).  Additionally, it requires assumptions that the runtime is consistently referring to the theatrical edition of these movies.} \\
    \bottomrule
    \end{tabularx}
    \label{tab:implicit_examples}
\end{table*}

==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/qc_stats.tex <==
\begin{table*}
    \caption{Quality measure on samples of annotations for conversational QA, summarization, and table-to-text tasks. Snapshots represent consecutive annotation sprints with individual annotator judgements (Ann) replicated at 5 per task. A sample (\textit{Smpl}) of each snapshot was evaluated by a project lead on the annotator team. The quality of annotations (\textit{Qual}) was assessed over a varying number of snapshots for each task. The evaluated annotations exclude flagged tasks.}
    \begin{tabular*}{\textwidth}{l|lll|lll|lll}
    \toprule
    &\multicolumn{3}{c|}{Conversational QA}
    &\multicolumn{3}{c|}{Summarization}
    &\multicolumn{3}{c}{Table-to-Text}\\
        Snapshot & Ann & Smpl & Qual & Ann & Smpl & Qual & Ann & Smpl & Qual\\
        \midrule
        1 & 642 & .04 & 1.00 & 88 & .06 & .67 & 261 & .08 & 1.00 \\
        2 & 726 & .05 & 1.00 & 339 & .06 & .87 & 2,518 & .19 & .96 \\
        3 & 1,895 & .03 & 1.00 & 469 & .10 & .94 & 2,463 & .30 & .97 \\
        4 & 2,520 & .04 & .97 & 682 & .08 & 1.00 & 1,151 & .34 & .96 \\
        5 &-&-&-& 608 & .08 & 1.00 & 849 & .30 & .94 \\
        6 &-&-&-& 652 & .08 & 1.00 &-&-&- \\
        7 &-&-&-& 928 & .03 & 1.00 &-&-&- \\
        \midrule
        \emph{Total} & 5,783 & .04 & .99 & 3,766 & .07 & .98 & 7,242 & .26 & .96 \\
        \bottomrule
    \end{tabular*}
    \label{tab:qc_stats}
\end{table*}

==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/qrecc_results_table.tex <==
\begin{table*}
    \caption{Results of human study on 200 examples from QReCC test set (randomly sampled from set of examples where conversation length $\leq5$ turns). PT= pretrained model, FT=fine-tuned on QReCC training data.}
    \begin{tabular*}{\textwidth}{l l | l l}
        \toprule
        Model & Size& Int & AIS  \\
        \midrule
        T5-PT (with Evidence) & Small & 43.0$^*$ & 82.6\\
        & Base & 47.0$^*$ & 69.1$^*$\\
        T5-FT (no Evidence) & Small & 57.8$^*$ & 25.2$^*$\\
        & Base & 59.8$^*$ & 21.8$^*$\\
        T5-FT (with Evidence) & Small & 99.0 & 87.9\\
        & Base & 98.0 & 87.2 \\
        \midrule
        {\it Reference}& & 99.0 & 87.8 \\
        \bottomrule
    \end{tabular*} \\
    \label{tab:qrecc}
    \tabnote{\footnotesize{* Indicates that the result is significantly lower than the \textbf{highest score} in the column (with $p<0.01$).}}
\end{table*}

==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/tasks_table.tex <==
\begin{table*}
    \caption{Summary of tasks used in human annotation study.}
    \begin{tabularx}{\textwidth}{X >{\raggedright}X X >{\raggedright\arraybackslash}X X}
        \toprule
        Task & Dataset & $C$ & $P$ & $S$ \\
        \midrule
        Conversational QA & QReCC \cite{qrecc} & Conversational History & Retrieved Document & Response \\
        \midrule
        Conversational QA & Wizard of Wikipedia \cite{dinan2019wizard} & Conversational History & Retrieved Fact & Response \\
        \midrule
        Summarization & CNN/DM \cite{cnndm} & N/A & Source Article & Summary \\
        \midrule
        Table-To-Text & ToTTo \cite{parikh-etal-2020-totto} & N/A & Table, Table Description & Caption \\
        \bottomrule
    \end{tabularx}
    \label{tab:tasks}
\end{table*}

==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/totto_results_table.tex <==
\begin{table*}
    \caption{Results of human study on 200 examples from ToTTo test set (model output) and development set (ground-truth references).}
    \begin{tabular*}{\textwidth}{l|lll}
        \toprule
        Model & Flag & Int & AIS  \\
        \midrule
        ByT5-Base & 0.0 & 78.9* & 88.5\\
        ByT5-XL & 0.0 & 79.5* & 86.2\\
        T5-Small & 3.0 & 86.5 &88.6\\
        T5-Base & 5.0 & 91.1 & 86.6 \\
        T5-XL & 6.0 & 89.4 & 85.1*\\
        \midrule
        {\it Reference} &0.0& 83.9 & 91.0 \\
        \bottomrule
    \end{tabular*}\\
    \tabnote{\footnotesize{* Indicates that the result is significantly lower than the \textbf{highest score} in the column (with $p<0.01$)}}
    \label{tab:totto}
\end{table*}

==> AIS Paper (Arxiv Copy) - July 19, 2022/tables/wow_results_table.tex <==
\begin{table*}
    \caption{Results of human study on 200 examples from Wizard of Wikipedia test set \citep{dinan2019wizard} (the seen topic split, using only conversation turns where the previous turn has a question mark).}
    \begin{tabular*}{\textwidth}{l | l l l}
        \toprule
        Model & Flag & Int & AIS   \\
        \midrule
        WoW Baseline \cite{dinan2019wizard} &4.0 & 84.4$^*$ & 19.8$^*$ \\
        Dodeca \cite{dodeca} &  8.5&100.0 & 60.1$^*$\\
        T5 \cite{t5ppr} & 5.5& 98.4 & 39.8$^*$ \\
        T5 (with Controls) \cite{rashkinetal} &7.5& 99.5 & 92.4 \\
        \midrule
        {\it Reference} & 4.0 &100.0 & 15.6$^*$ \\
        \bottomrule
    \end{tabular*}\\
    \tabnote{\footnotesize{* Indicates that the result is significantly lower than the \textbf{highest score} in the column (with $p<0.01$).}}
    \label{tab:wow}
\end{table*}
